How to prevent type-flaw attacks on security protocols under algebraic properties

Type-flaw attacks upon security protocols wherein agents are led to misinterpret message types have been reported frequently in the literature. Preventing them is crucial for protocol security and verification. Heather et al. proved that tagging every message field with it's type prevents all type-flaw attacks under a free message algebra and perfect encryption system. In this paper, we prove that type-flaw attacks can be prevented with the same technique even under the ACUN algebraic properties of XOR which is commonly used in "real-world" protocols such as SSL 3.0. Our proof method is general and can be easily extended to other monoidal operators that possess properties such as Inverse and Idempotence as well. We also discuss how tagging could be used to prevent type-flaw attacks under other properties such as associativity of pairing, commutative encryption, prefix property and homomorphic encryption.

==> app-proofs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%    PROOFS FOR LEMMAS		%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proofs}\label{sa.proofs}	

%\subsection{Lemmas}
The following lemma proves that the reduction rules corresponding to standard attacker inferences always add existing subterms to the term set of the original constraint.

\begin{lemma}[Rules in $R$ always produce subterms]\label{la.produce-subt}

	If a rule in $R$ is applied to a constraint $c = m~:~T$ such that $c$ is reduced to $m~:~T \cup t$, then $t \sqsubset T$.

\end{lemma}
\begin{proof}

	Only ({\em pdec}), ({\em sdec}), ({\em split}), ({\em ksub}) apply on $T$. 
	
	\begin{itemize}
	
		\item ({\em split}) splits $[t_1, t_2] \in T$ into $t_1$ and $t_2$ which are subterms;
		\item ({\em ksub}) only instantiates $k$ in $[t]^{\leftrightarrow}_k$ unifying it with $\mi{pk}(\epsilon)$;
		\item ({\em pdec}) derives $t$ from $[t]^{\to}_k$ which is a subterm;
		\item ({\em sdec}) splits $[t]^{\leftrightarrow}_k \in T$ into $t$ and $k$ where $t$ is a subterm and $k$ is also a subterm since it is derived from $T \cup [t]^{\leftrightarrow}_k$ by satisfying $k~:~T \cup [t]^{\leftrightarrow}_k$ before it is added to $T \cup t$ which is only possible if $k$ was a subterm of $T$.
	
	\end{itemize}


\end{proof}

The following lemma proves that inserting distinct constants into distinct parametric terms of a protocol ensures that the terms remain non-unifiable even after the protocol is instantiated into a semi-bundle:

\begin{lemma}[NUT guarantees non-unifiability in semi-bundles]\label{la.nut}

	If two terms $t_1$, $t_2$ in a semi-bundle $S$ from an \textsf{NUT}-Satisfying protocol  $P$ are such that $t_1 = \sigma^h_a t'_1$ and $t_2 = \sigma^h_b t'_2$ where $\sigma^h_a \neq \sigma^h_b$ and $\{ \sigma^h_a, \sigma^h_b \} \subseteq \sigma^H_S$ and $S = \sigma^H_S P$, $t'_1, t'_2 \in P$, and $t'_1 \neq t'_2$, then $t_1 \not\approx t_2$.

\end{lemma}

\begin{proof}

If $t'_1 \neq t'_2$, it implies that $t'_1 \not\approx t'_2$ from Def.~\ref{d.Mu-NUT}. So the hypothesis is $t'_1 \not\approx t'_2 \Rightarrow t_1 \not\approx t_2$ since $t'_1$, $t'_2$ are parametric terms, they contain only variables or constants. Hence,  the unifier when $t'_1$ and $t'_2$ are unified would be the most general unifier (mgu). Since this mgu itself is not possible, a more specific unifier that would be obtained by unifying $t_1$ and $t_2$ (which have lesser variables compared to $t'_1$ and $t'_2$) is not possible as well (recall that every unifier is an extension of the mgu from the definition of unification, Def.~\ref{d.unif}).

\end{proof}

The following lemma proves that unification in a semi-bundle from a {\sf NUT}-Satisfying protocol always returns well-typed unifiers when terms are formed using the term algebra in Def.~\ref{d.term-algebra} (standard theory).

\begin{lemma}[Necessarily well-typed unifiers]\label{la.well-typed}

 Let $S$ be a semi-bundle from a {\sf NUT}-Satisfying protocol and let $t, t' \in S$ for a semi-bundle $S$ such that $t = \sigma^h_{s} x$ and $t' = \sigma^h_{s'} x$ for some $s, s' \in S$. Then, $\text{\sf well-typed}(\tau)$ where $\text{mgu}(t,t') = \tau$.

\end{lemma}

\begin{proof}

Firstly note that $t$ cannot be a variable since procedure {\bf P} applies a reduction rule on the first constraint that does not have a variable on the left. Also, $t'$ cannot be a variable since {\bf P} applies rule ({\em elim}) to eliminate all variables in the term set of the active constraint before applying any other rule. 

Obviously, $t$ or $t'$ cannot be atoms as well. This leaves us with the case where both $t$ and $t'$ belong to $\mi{CT}(S)$.

From Assumption \ref{a.well-typed}, we have $\text{\sf well-typed}(\sigma^{h}_{s}) \wedge \text{\sf well-typed}(\sigma^h_{s'})$.  Let $x = f(x_1, \ldots, x_n)$ for some free function $f$ where $f$ is encryption, hash, or sig. Since $t \approx t'$ and since $t, t'$ can occur on a node with `$-$' and `$+$' signs respectively, for each $x_i$ ($i = 1~\text{to}~n$) only one of either $\sigma^h_s$ or $\sigma^h_{s'}$ define substitutions for $x_i$ and the other does \underline{not}. Let $\sigma^h_{s}$ be the one which defines substitution for $x_i$. Then $\text{\sf well-typed}(\sigma^h_{s} x_i)$ and $\sigma^h_{s'}$ does not define a substitution for $x_i$ and further, the unifier for $\sigma^h_{s} x_i$ and $\sigma^h_{s'} x_i$ will be $\sigma^h_{s}$ which is well-typed. Similarly for all $i = 1~\text{to}~n$ (and recursively to any subterms of $x_i$). Hence, $\text{\sf well-typed}(\tau)$.

\end{proof}

We reprove the above lemma under equational unification corresponding to the {\sf ACUN} theory. A similar proof can be given for {\sf ACUIdem} and {\sf ACUInv}. The {\sf ACUN} theory $E_{\msf{ACUN}}$ is described by the equations below:

$a \oplus [b \oplus c] = [a \oplus b] \oplus c$ (Associativity), $a \oplus b = b \oplus a$ (Commutativity), $a \oplus 0 = a$ (existence of Unity), $a \oplus a = 0$ (Nilpotence).

Let the standard theory $E_{\msf{STD}}$ be the term algebra defined in Def.~\ref{d.term-algebra}.

Chevalier's extension of the constraint solving procedure {\bf P} under $E_{\msf{STD}}$ to $\mbf{P_{\oplus}}$ under $E_{\msf{STD}} \cup E_{\msf{ACUN}}$ consisted of mainly the following two additional reduction rules to $R$:

\begin{center}
       \[ \frac{C_<,~t_1 \oplus \ldots \oplus t_n : T,~C_>;~\sigma}{ C_<, t_1 : T_, \ldots, t_n : T, C_>;\sigma }~~~(\mi{XOR_L})  \]

       \[ \frac{C_<, m : T \cup \{t_1, \ldots , t_n\}, C_>; \sigma}{ C_<, m : T \cup t_1 \oplus \ldots \oplus t_n, C_>;\sigma }~~~(\mi{XOR_R})  \]

\end{center}

As an extension to {\sf NUT} for $(E_{\msf{STD}} \cup E_{\msf{ACUN}})$, we will require that a {\sf pair} tag or an appropriate tag indicating the type of the sequence will be included for a sequence of terms joined by the \texttt{XOR} operator when brackets are used to segregate them. For example, $[[\msf{nonce},n_a]\oplus[\msf{agent},A]]\oplus[\msf{key},K]$ is tagged as $[\msf{nonce\oplus agent},[\msf{nonce},n_a] \oplus [\msf{agent},A]]\oplus [\msf{key},K]$. Such tagging voids the associativity property of $\oplus$.

We will also require that every individual term in a sequence of terms connected with the $\oplus$ operator is type-tagged.

For the lemma below, we assume that algorithms $A_{\msf{STD}}$ for unification of problems in $E_{\msf{STD}}$ and $A_{\msf{ACUN}}$ for $E_{\msf{ACUN}}$ described in \cite{Tuengerthal-TR-2006} are used, while the combination algorithm of Baader and Schulz (also described in \cite{Tuengerthal-TR-2006}) is used for the combined unification of $(E_{\msf{STD}} \cup E_{\msf{ACUN}})$. We will assume that the reader is familiar with the combination algorithm of \cite{BS96}. While Tuengerthal's algorithm offers practical and efficient extensions for the non-deterministic algorithm of \cite{BS96}, the extensions need not be considered in our proof since they do not produce any new unifier (but only optimize finding the ones that can be identified by \cite{BS96}). The algorithm of \cite{BS96} on the other hand offers a simple and clean presentation that is useful and sufficient for our proofs, despite its non-deterministic approach. Furthermore, it is a general combination method for any two theories, not merely $E_{\msf{STD}} \cup E_{\msf{ACUN}}$. Hence, it allows us to extrapolate our results to other similar combinations as well such as $E_{\msf{STD}} \cup E_{\msf{ACUInv}}$ and $E_{\msf{STD}} \cup E_{\msf{ACUIdem}}$.

The intuition behind the proof for the lemma is as follows: informally, the problem of unification of two terms under the combined theory of $(E_{\msf{STD}} \cup E_{\msf{ACUN}})$ must first result in subproblems that are purely in $E_{\msf{STD}}$ or purely in $E_{\msf{ACUN}}$ according to Baader-Schulz algorithm. Now $E_{\msf{STD}}$ problems result in a well-typed unifier from Lemma~\ref{la.well-typed}. 

This leaves us with $E_{\msf{ACUN}}$ problems. These problems will have a unifier only if the \texttt{XO}R terms contain variables. However, according to our extended requirement of {\sf NUT} above, no protocol term has an \texttt{XOR} term with an untagged variable. Further, the \texttt{XOR} terms produced by $\mbf{P_{\oplus}}$ in the term set of a constraint cannot contain variables either since like in {\bf P}, the rule ({\em elim}) eliminates any stand-alone variables in a term set before applying any other rule. Thus, algorithm $A_{\msf{ACUN}}$ returns an empty unifier. Unification of $E_{\msf{ACUN}}$ problems only happens when two standard terms that were replaced by variables belong to the same equivalence class can be unified with $A_{\msf{STD}}$ and could thus be canceled. That unifier from $A_{\msf{STD}}$ is again well-typed from Lemma~\ref{la.well-typed}. 

In summary, the unifier for a problem in  $(E_{\msf{STD}} \cup E_{\msf{ACUN}})$ under the extended requirement on {\sf NUT} is only from applying $A_{\msf{STD}}$ and is always well-typed.

\begin{lemma}[Necessarily well-typed unifiers under $E = E_{\msf{STD}} \cup E_{\msf{ACUN}}$]\label{la.well-typed-xor}

Let $C$ be a constraint sequence from a semi-bundle $S$ from an \textsf{NUT}-Satisfying protocol and let $m~:~T$ be the active constraint when $C$ is being solved using $\mbf{P_{\oplus}}$. Then, for each $\tau = \text{mgu}(m,t)$, where $t \in T$, $\tau$ is well-typed.

\end{lemma}

\begin{proof}

Following the combination algorithm of \cite{BS96} described in \cite{Tuengerthal-TR-2006}, let the initial problem of $\Gamma = \{ t \stackrel{?}{\approx_E} t' \}$ be reduced to $(\Gamma',<,p)$ where 

\begin{itemize}

	\item $\Gamma'$ is a set of unification problems $\{ s_1 					\stackrel{?}{\approx} t_1, \ldots, s_n 											\stackrel{?}{\approx} t_n \}$;
	\item Let $\Gamma'$ be pure with every $t_1 											\approx_E t_2 \in \Gamma'$ have $t_1$, $t_2$  							formed purely from operator $\oplus$ on $0$, 								constants and variables or from the standard 								theory in the term algebra defined in 											Def.~\ref{d.term-algebra};
	\item $<$ is a linear ordering on variables such that if 					$X < Y$ then $Y$ does not occur as a subterm of the 				instantiation of $X$;
	\item $p$ is a partition $\{ V_1, V_2 \}$ on the set of 					all variables $V$ such that $V_2$ are treated as 						constants when $A_{\msf{STD}}$ is applied and $V_1$ 				are constants when $A_{\msf{ACUN}}$ is applied;
	\item Let another partition $p'$ of variables identifies 					equivalence classes of $V$ where every class in a 					partition is replaced with a representative and 						where members of the class are unifiable; 	

\end{itemize}

Let the combined unifier of $\sigma_{\msf{STD}}$ and $\sigma_{\msf{ACUN}}$ denoted $\sigma_{STD} \odot \sigma_{ACUN} = \sigma$ which is obtained by applying \cite[Def.~9]{Tuengerthal-TR-2006}; i.e., by induction on $<$. Our aim is to prove that every $\sigma$ obtained for different combinations of $<, p, p'$ is well-typed. 

Let us examine the possible forms of problem elements in $\Gamma'$ (below note that $t \stackrel{?}{\approx_E} t'$ is the main unification problem $\Gamma$ and $\Gamma'$ is a set of subproblems of $\Gamma$ after purification):

\begin{description}

	\item[$\msf{STD}$ theory:] $t_1 \approx_{\msf{STD}} t_2$ 				where 
				\begin{enumerate}
						\item $t_1$ is some $f(t'_1)$ and $t_2$ is some 									$f(t'_2)$, with $f$ an encryption, hash 										or signature; Every such problem returns 										a well-typed unifier from 																	Lemma~\ref{la.well-typed}.
						\item either $t_1$ or $t_2$ is a new variable 										belonging to $V$; there is no unifier to 										existing variables in $t$ or $t'$ here.
				\end{enumerate}
	
	\item[$\msf{ACUN}$ theory:] $t_1 \oplus t_2 \oplus \ldots 								\oplus t_m \stackrel{?}{\approx_{\msf{ACUN}}} t'_1 \oplus 									t'_2 \oplus \ldots \oplus t'_n$ where each of 								$t_i$ ($i$ = 1 to $m$) and $t'_i$ ($i$ = 1 									to $n$) is a constant or a new variable in $V$.  						The reason is as follows: according to the 									requirement on protocol messages, if $t$ is a 							subterm of the semi-bundle, then no $t_i$ can be an 				untagged variable. Also, if $t'$ is in the term set 				of a constraint, then no $t'_i$ is a variable, 							since $\mbf{P_{\oplus}}$ applies rule ({\em elim}) 					eliminating all stand-alone variables before 								applying any other rule. Lastly, the new variables 					in $t$ and $t'$ would be other problems in 									$\Gamma'$ of the form $X = 																	[\msf{tag},\mathrm{t^{''}}]$ where $X$ is the new 					variable, $\msf{tag}$ is a constant and $t^{''}$ is 				any term. These new variables are treated as 								constants when applying $A_{\msf{ACUN}}$. With all 					constants in $t$ and $t'$, $A_{\msf{ACUN}}$ that 						would normally return a set of $0$ substitutions 						for some variables, returns an empty set of 								substitutions answering that $t$ and $t'$ are 							equivalent (if they are). 
	
\end{description}	

		In addition to the above, we need to consider another 			important case: if $t_1$ and $t_2$ are two new 							variables in the variable identification partition 					$p'$. However, since both are problems in $\Gamma'$ 				are such that they map to a tagged pair or compound 				term in the standard theory, their unifier is once 					again well-typed from Lemma~\ref{la.well-typed}. Note 			that we do not need to consider where either $t_1$ or 			$t_2$ is an existing variable since variables in {\sf 			ACUN} problems are necessarily new variables as 						explained above.

\end{proof}

\begin{corollary}\label{c.other-theories}

A similar argument applies in the case of other monoidal operators possessing equations {\sf Idempotency (Id)}  or {\sf Inverse (In)} in addition to {\sf ACUN}. When the combination algorithm of Baader \& Schulz is applied for $E_{\msf{STD}} \cup E_{\msf{T}}$ where $T$ is a theory with any, some or all of {\sf A, C, U, N, Id, In}, the algorithm for $\msf{T}$, say $A_{\msf{T}}$ will return an empty substitution when the operator with theory is so used in the protocol such that every term is type-tagged. Consequently, the unifier for the combined unification problem will only have substitutions from $A_{\msf{STD}}$ which is well-typed from Lemma~\ref{la.well-typed}.


\end{corollary}

==> app-prot-model.tex <==
\section{Constraint Solving}\label{sa.prot-model}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  Reduction Procedure, P [MS01]   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Constraint Satisfaction Procedure \textbf{P}~\cite{MS01}}\label{ssa.redn-proc}

\begin{center}
 \begin{tabbing}
  \= ~~~$C :=$~initial constraint sequence \\
  \> ~~~$\sigma := 0$ \\
  \> ~~~\texttt{repeat} \\
  \> ~~~~~~ \texttt{let} $c^* = m : T$ be \= the constraint in $C$ \\
  \> \>  s.t. $m$ is not a variable \\
  \> ~~~~~~ \texttt{if} $c^*$ \= not found \\
  \> \> \texttt{output} \textbf{Satisfiable!} \\
  \> ~~~~~~apply rule \textit{(elim)} to $c^*$ until no longer applicable \\
  \> ~~~~~~$\forall r \in R$ \\
  \> ~~~~~~~~~\texttt{if} $r$ \= is applicable to $C$ \\
  \> \> $\langle C';\sigma'\rangle := r(C;\sigma)$ \\
  \> \> create node with $C'$; add $C \to C'$ edge \\
  \> \> push $\langle C'; \sigma' \rangle$ \\
  \> ~~~~~~~~~$\langle C;\sigma\rangle :=$ \texttt{pop} \\
  \> ~~~\texttt{until emptystack}  
 \end{tabbing}
\end{center}



==> decide.tex <==
\section{Decidability}\label{s.decidability}

Decidability is usually assumed for protocol security if type-flaw attacks can be prevented; i.e., if analysis can be restricted to well-typed runs only. Below we describe how this does not hold under inferences that break the perfect encryption assumptions (e.g. using weak passwords). 

%\subsection{Password protocols}\label{ss.passwd}

It is well-known that weak secrets such as human-chosen passwords can be subject to \emph{guessing attacks} where the key is guessed and verified by using the messages in the protocol \cite{GMLN93,LGSN89}. 

Consider an inference that is possible when passwords or weak keys are used \cite{Lowe02}:

\[ \{ [t_1, t_2]^{\leftrightarrow}_{\mi{passwd}}, [t_1, t'_2]^{\leftrightarrow}_{\mi{passwd}} \} \vdash \mi{passwd} \]
 
This inference is not strictly due to any algebraic properties of the operators including the ciphers, but nevertheless possible when the key is from a short list of guesses.


The following example illustrates that non-unifiability does not necessarily guarantee decidability for password protocols when guessing attacks are possible even when type-flaw attacks are avoided\footnote{The example is motivated by Gong's demonstration protocol \cite{LGSN89} and the corresponding attack by the same authors in \cite{GMLN93}.}. 

Consider the protocol below:

\begin{center}
\begin{tabular}{ll}

Msg 1. $A \to B : [1, A, B, N_A]^{\to}_{pk(B)}$ \\

Msg 2. $B \to A : [ N_A,K ]^{\leftrightarrow}_{\mi{passwd}(A,B)}$\\

\end{tabular}
\end{center}

An attack is possible on this protocol involving two runs:

\begin{center}
\begin{tabular}{ll}

Msg $\alpha$.1. $a \to b : [1, a, b, n_a]^{\to}_{pk(b)}$ \\

Msg $\alpha$.2. $b \to a : [ n_a,k ]^{\leftrightarrow}_{\mi{passwd}(a,b)}$\\

Msg $\beta$.1. $i(a) \to b : [1, a, b, n_a]^{\to}_{pk(b)}$~~~~(replaying Msg $\alpha$.1) \\

Msg $\beta$.2. $b \to i(a) : [ n_a,k' ]^{\leftrightarrow}_{\mi{passwd}(a,b)}$\\

\end{tabular}
\end{center}

In this attack, an attacker eavesdrops on a legitimate conversation between $a$ and $b$ (run $\alpha$). He then replays their Msg 1 in another run $\beta$ in which he spoofs as $a$ to $b$. He then captures $[ n_a, k ]^{\leftrightarrow}_{\mi{passwd}(a,b)}$ in $\alpha$ and $[ n_a, k' ]^{\leftrightarrow}_{\mi{passwd}(a,b)}$ in $\beta$ (notice that the nonce $n_a$ remains the same but the key is a new, fresh key $k'$). Finally, he guesses the password, decrypts both terms and checks that $n_a$ exists in both terms (which is an unlikely coincidence) to verify the guess. Clearly, this attack conforms to  the inference for guessing attacks given above.

%It is trivial to see that the protocol obeys non-unifiability, yet there is an attack involving more than one run, but not on an isolated run. Thus, tagging does not guarantee decidability on password protocols.

It is interesting to note that this is not a type-flaw attack. The guessing attack inference works even on well-typed runs. However, it renders protocol security undecidable. This points to an interesting concept that even if type-flaw attacks can be prevented, protocol security could still be undecidable, contrary to the popular supposition; for instance in \cite{RS-FST03} decidability is proven by showing that analysis could be reduced to well-typed runs only, claiming that security is then decidable.

\begin{lesson}[Absence of type-flaw attacks does not guarantee decidability]\label{le.decidability}
	The lesson here to the protocol analyst is that decidability of protocol security is not guaranteed under the various algebraic properties we have considered in this paper including the free algebra preserving (e.g. Prefix property) and the non-free algebras (e.g. monoidal theories), even if tagging can prevent type-flaw attacks under those theories. Decidability results for tagged protocols under extended theories is an open problem.
\end{lesson}

==> extend.tex <==
\section{Extending to algebraic properties}\label{s.extend}

Similar to Heather et al.'s results, the previous section assumed that encryption is perfect and the algebra is free. Let us examine how the key aspects of the main result (Lemmas \ref{l.produce-subt}, \ref{l.nut}, \ref{l.well-typed}) are affected when we extend the message algebra which might break these assumptions.


\subsection{Properties breaking the perfect encryption assumption}\label{ss.Prefix-RSA}

We first consider algebraic properties that lead to cryptosystem weaknesses, without altering the freeness of the message algebra.
These weaknesses produce non-subterms, obviously violate Lemma~\ref{l.produce-subt}, and consequently Theorem~\ref{t.type-flaw}.

\subsubsection*{Prefix property.} The Prefix property is obeyed by block ciphering techniques such as CBC and ECB. This property leads  the attacker to infer $[m]^{\leftrightarrow}_k$ (a non-subterm) from $[m,n]^{\leftrightarrow}_k$ thereby invalidating Lemma~\ref{l.produce-subt}.

Consider the Woo and Lam $\pi_1$ protocol modified by inserting component numbers following Heather et al.'s suggestion:

\begin{center}
\begin{tabular}{ll}

Msg 1. $a \to b : a$ \\
Msg 2. $b \to a : n_b$ \\
Msg 3. $a \to b : [a, b, n_b, 1]^{\leftrightarrow}_{\mi{sh}(a,s)}$ \\
Msg 4. $b \to s : [a, b, [a, b, n_b, 1]^{\leftrightarrow}_{\mi{sh}(a,s)}, 2]^{\leftrightarrow}_{\mi{sh}(b,s)}$ \\
Msg 5. $s \to b : [a, b, n_b, 3]^{\leftrightarrow}_{\mi{sh}(b,s)}$

\end{tabular}
\end{center}

$sh(x,y)$ represents a shared-key between agents $x$ and $y$. 
We presented a type-flaw attack on this protocol in \cite{MA03} even when it uses Heather et al's scheme if the Prefix property is exploited:

\begin{center}
\begin{tabular}{ll}

Msg 1. $a \to b : a$ \\
Msg 2. $b \to a : n_b$ \\
Msg 3. $I(a) \to b : [n_b, 3]$ /* In place of $[a, b, n_b, 1]_{\mi{sh}(a,s)}$ */ \\
Msg 4. $b \to I(s) : [a, b, [n_b, 3], 2]^{\leftrightarrow}_{\mi{sh}(b,s)}$ \\
Msg 5. $I(s) \to b : [a, b, n_b, 3]^{\leftrightarrow}_{\mi{sh}(b,s)}$ /* using CBC inf rule on Msg 4. */ \\

\end{tabular}
\end{center}

This attack works because, an attacker can infer $[a, b, n_b, 3]^{\leftrightarrow}_{\mi{sh}(b,s)}$ from Msg~4 ($[a, b, [n_b, 3], 2]^{\leftrightarrow}_{\mi{sh}(b,s)}$) exploiting the Prefix property.

Will type-tagging prevent this attack? To find out, we need to examine if type-tagging can prevent Msg~5 to be inferred from Msg~4. Under type-tagging, Msg~4 would resemble $[\msf{Msg4Type}, [\msf{agent},a], [\msf{agent},b], \ldots ]^{\leftrightarrow}_{\mi{sh}(b,s)}$ and Msg~5 would resemble  $[\msf{Msg5Type}, [\msf{agent},a], [\msf{agent},b], \ldots ]_{\mi{sh}(b,s)}$. It can be easily seen that even under the Prefix property, Msg~5 cannot be derived, thanks to the tag $\msf{Msg4Type}$ inside Msg~4. 

Note that placing the component number `2' and `3' respectively in Msg~4 and 5 at the beginning of the concatenations will also prevent this attack, but a similar attack would be possible with such a placement under the ``Suffix property" that allows $[n]_k$ to be inferred from $[m,n]_k$. We leave it to the reader to check this.

\noindent
Our observation can be framed as the following principle for the protocol designer:

\begin{center}
\begin{tabular}{|l|}
\hline

\parbox[3,3]{4in}{\begin{lesson}[Placement of tags]\label{le.placement}
If ciphering techniques are not guaranteed to be perfect when a protocol is implemented, it would be prudent to place tags such that non-subterms cannot be inferred that could unify with other messages expected by agents.
\end{lesson}
}\\

\hline

\end{tabular}
\end{center}

\subsubsection*{Homomorphism of Encryptions.}
With this property, it would be possible to infer the non-subterms  $[m]_k$, and $[n]_k$ from $[m,n]_k$. Obviously, this is stronger than the Prefix property, but both component numbering and type-tagging could be implemented. 

The ``$\msf{pair}$" tag assumed to contain within parentheses cannot void this inference. For instance, a term $[[\msf{type_1},t_1],[\msf{type_2},t_2]]_k$ can still yield the non-subterms $[\msf{type_1},t_1]_k$, and $[\msf{type_2},t_2]_k$. Even with component numbering, a term such as $[1,[t_1,t_2]]_k$ can broken down into $[1]_k$, and $[t_1,t_2]_k$.

With a range of such non-subterm encryptions to infer, it can be easily seen that neither component numbers, nor type-tags, no matter how they are placed, can prevent the attack on the Woo and Lam protocol above under this inference. 

In particular, if the plaintext block length equals the length of a nonce or agent, then the attacker can infer $[a]_{\mi{sh}(b,s)}$, $[b]_{\mi{sh}(b,s)}$, $[n_b]_{\mi{sh}(b,s)}$ easily from Msg~4 under any tagging. He can then replay Msg~5 by stitching these together.

However, this inference is only possible under an extremely weak system such as ECB, so a realistic threat in real-world situations is unlikely.

\subsubsection*{Low-exponent RSA weakness.} Another unrealistic, but academically interesting inference is the one on RSA shown by Coppersmith \emph{et al.}~\cite{CFPR96}: \\

 $ \{ [a, [x, b]]^{\rightarrow}_k, [c, [x,d]]^{\rightarrow}_k, a, b, c, d \} \vdash x, \text{where}~~a \neq c \vee b \neq d$. \\
 
Clearly, since this inference produces a subterm (`$x$'), the main result stands tall in its presence and no type-flaw attacks can be possible if the protocol obeys {\sf NUT}. \\


%However, this inference gives a nice example to show that the absence of type-flaw attacks does not guarantee decidability of protocol security when perfect encryption is broken. Consider for example, the message $[N_A,N_B,B]_{\mi{pk}(B)}$ in a protocol can lead to $[n_a,n_b,b]_{\mi{pk}(b)}$ and $[n'_a,n_b,B]_{\mi{pk}(B)}$:




\subsection{Properties breaking the free algebra assumption}\label{ss.break-free}

Some algebraic properties break the free algebra assumption by allowing equations between terms. These make equational unification necessary for complete analysis, thereby affecting Lemma~\ref{l.well-typed}. We will consider these now and see if we can tag terms so that Lemma~\ref{l.well-typed} withstands the properties.

\subsubsection*{Associativity of Pairing.}
This property allows the equation $[a,[b,c]] = [[a,b],c]$. Both type-tagging and component numbering can be implemented as usual. For instance, the term $[n_a,[a,N_B]]_{\mi{pk}(B)}$ can be transformed into $[1,n_a,[a,N_B]]_{\mi{pk}(B)}$ or $[[\msf{nonce},n_a],[[\msf{agent},a],[\msf{nonce},N_B]]]_{\mi{pk}(B)}$. 

It is trivial to see that only unification needs to be considered under this property, if we assume perfect encryption. Component numbering cannot prevent ill-typed unifiers. A simple example can prove this: $[1,A,[b,c],d]$ can be unified using $[1,[a,B],C,d]$, with $\sigma =  \{ [a,B]/A, [b,c]/C, d/D \}$. Obviously, $\sigma$ is ill-typed.

Can type-tagging prevent ill-typed unifiers? Yes. For example, \\
$[[\msf{agent},A],[[\msf{nonce},b],[\msf{agent},c]],[\msf{key},d]]$ cannot be unified with \\ $[[[\msf{agent},a],[\msf{nonce},B]],[\msf{agent},C],[\msf{key},D]]$ even under associativity, as long as a ``$\msf{pair}$" tag is included to indicate pairs (assumed to contain within  parentheses). It would be straightforward to prove this claim formally.

%The lesson to learn here is that replacing type-tags with component numbers is \underline{not} a ``safe simplifying transformation" under some properties in contrast to that stated in \cite{HLS03}\footnote{To be fair to Heather et al., let us acknowledge that most likely they did not have such algebraic properties in mind when they made that claim.}. 

We can frame this observation as the following principle:

\begin{center}
\begin{tabular}{|l|}
\hline

\parbox[3,3]{4in}{
%\begin{quote}
\begin{lesson}[``Unsafe" simplification transformations]\label{le.unsafe}

Security is not preserved under simplified tagging schemes in the presence of algebraic properties. It would be prudent to properly examine this in order to not result in over simplifications.

\end{lesson}
%\end{quote}
}\\

\hline

\end{tabular}
\end{center}



\subsubsection*{Commutativity of Encryptions.}
This property allows the equation $[[t]^{\to}_{k_1}]^{\to}_{k_2} = [[t]^{\to}_{k_2}]^{\to}_{k_1}$. Both component numbering and type-tagging can be easily implemented and they both would render this equation inapplicable. For instance, $[\msf{penc},[\msf{nonce},n_a]^{\to}_{k_1}]^{\to}_{k_2}$ cannot equal $[\msf{penc},[\msf{nonce},n_a]^{\to}_{k_2}]^{\to}_{k_1}$ due to the tag $\msf{penc}$ inside.

However, when combined with homomorphic encryption discussed above, the equation can come to life even with tags: Consider $[c_1,[c_2,t]^{\to}_{k_1}]^{\to}_{k_2}$ which can equal $[[c_1]_{k_2},[[c_2,t]_{k_1}]_{k_2}]$ due to homomorphism and 
$[[c_2,t]_{k_1}]_{k_2}$ can then equal $[[c_2,t]_{k_2}]_{k_1}$.

If $k_1$ can be unified with $\mi{pk}(\epsilon)$, then the commutative property can produce $[c_2,t]_{k_2}$ which is another non-subterm in addition to $[[c_2,t]_{k_2}]_{k_1}$ which voids Lemma~\ref{l.produce-subt}. This observation prompts another principle:

\begin{center}
\begin{tabular}{|l|}
\hline

\parbox[3,3]{4in}{\begin{lesson}[Combination of properties]\label{le.combination}
	Tags might themselves void some properties. Also, properties that are harmless individually could be harmful in combination. It would be prudent to check for properties as a whole, not merely in isolation.
\end{lesson}
}\\

\hline

\end{tabular}
\end{center}

Although non-subterms $[c_2,t]_{k_2}$ and $[[c_2,t]_{k_2}]_{k_1}$ are produced when commutative and homomorphic encryptions are combined, they will not induce an ill-typed substitution when unified with a target term; due to component numbers, they can be unified only with other semi-terms that have been derived using the same parametric term. For instance, $[c_2,t]_{k_2}$ can only be unified with some $[c_2,t']_{k'}$ with $t$ the same type as $t'$ and $k_2$ the same type as $k'$. This is of course not true when component numbers are not included inside encryptions.

\subsubsection*{Monoidal theories.}\label{sss.monoidal} 
Following the definition of monoidal theories from \cite{CortierD07}, we can determine that 

\begin{itemize}

\item the theory {\sf ACU} over $\{ +, 0 \}$ where {\sf A} stands for associativity, {\sf C} for commutativity and {\sf U} for the existence of Unity is a monoidal theory;

\item the theories {\sf ACUIdem} and {\sf ACUN} where {\sf Idem} stands for Idempotence and {\sf N} for Nilpotence are also monoidal theories over $\{+,0\}$ and $\{\oplus,0\}$ respectively; 

\item the theory of Abelian Groups ({\sf AG} or {\sf ACUInv}) over $\{ +, -, 0 \}$ where {\sf Inv} stands for Inverse is also monoidal where $-$ is a unary operator.

\end{itemize}

We have already seen that associativity of pairing induces type-flaw attacks that can be prevented with only type-tagging but not component numbering. It is easy to see that the same is true even when considering associativity of a general operator using the examples $[1,[a.b].C]$ and $[2,A.[b.c]]$ or $[[[\msf{agent},a],[\msf{nonce},b]],[\msf{key},C]]$ and $[[\msf{agent},A],[[\msf{nonce},b],[\msf{key},c]]]$.

The same holds for commutativity as well: Consider $[1,n_a.B.a]$ unified with $[1,A.b.N_A]$ that results in an ill-typed unifier $\{ n_a/A, b/B, a/N_A \}$ but type-tagging does not allow such a unification and ensures well-typed unification. Consider the same example: $[\msf{nonce}.\msf{agent}.\msf{agent},[\msf{nonce},n_a].[\msf{agent},B].[\msf{agent},a]]$ cannot be unified with  $[\msf{nonce}.\msf{agent}.\msf{agent},[\msf{agent},A].[\msf{agent},b].[\msf{nonce},N_A]]$. 

Since type-tagging is unavoidable for {\sf A} and {\sf C}, let us examine how the other properties of {\sf Unity}, {\sf Idempotency}, {\sf Nilpotency} and {\sf Inverse} affect type-flaw attacks. Let us start with the {\sf ACUN} theory.


Consider the adapted version of the NSL protocol presented by Chevalier et al. in \cite{CKRT03}. We further modify it by type-tagging messages:


\begin{center}
\begin{tabular}{ll}

Msg 1. $A \to B : [[\msf{agent},A],[\msf{nonce},N_A]]^{\to}_{\mathit{pk}(B)}$ \\

Msg 2. $B \to A : [ [\msf{nonce}\oplus\msf{agent},N_A \oplus B],  [\msf{nonce},N_B] ] ]^{\to}_{\mathit{pk}(A)}$\\

Msg 3. $A \to B : [\msf{nonce},N_B]^{\to}_{pk(B)}$\\

\end{tabular}
\end{center}

A type-flaw attack is possible on this protocol despite the type-tagging (a similar attack is also possible with component numbering; see Appendix~\ref{sa.xor-attack}):

\begin{center}
\begin{tabular}{ll}

Msg $\alpha$.1. $a \to i : [ [\msf{agent}, a], [\msf{nonce},n_a] ]^{\to}_{\mathit{pk}(i)}$ \\

~~Msg $\beta$.1. $i(a) \to b : [ [\msf{agent}, a], [\msf{nonce}, n_a \oplus b \oplus i] ]^{\to}_{\mathit{pk}(b)}$ \\

~~Msg $\beta$.2. $b \to i(a) : [ [\msf{nonce} \oplus \msf{agent}, n_a \oplus b \oplus i \oplus b], [\msf{nonce},n_b]]^{\to}_{\mathit{pk}(a)}$ \\

Msg $\alpha$.2. $i  \to  a : [ [\msf{nonce} \oplus \msf{agent},n_a \oplus i], [\msf{nonce},n_b]]^{\to}_{\mathit{pk}(a)}$ \\

Msg $\alpha$.3. $a \to i : [\msf{nonce},n_b]^{\to}_{pk(i)}$\\

~~Msg $\beta$.3. $i(a) \to b : [\msf{nonce},n_b]^{\to}_{pk(b)}$\\


\end{tabular}
\end{center}

In this attack, $n_a \oplus b \oplus i \oplus b$ in Msg $\beta$.2 is reduced to $n_a \oplus i$ in Msg $\alpha$.2 by canceling `$b$' that is present twice in the expression.

Notice also the type-flaw in Msg $\beta$.1 by $i(a)$ sending $\msf{nonce} \oplus \msf{agent} \oplus \msf{agent}$ claiming it as a $\msf{nonce}$. This attack cannot exist without this type-flaw. Hence, this is strictly a type-flaw attack.

Under {\sf AG} (or {\sf ACUInv}) property, the same concepts apply: Neither type-tagging nor component numbering prevent type-flaw attacks under the {\sf Inverse} property which allows cancellation much like {\sf Nilpotence}. Consider operators $\{+,-\}$, where $+$ is binary addition, $-$ unary, and $0$ a constant. Then, if we change the $\oplus$ operator in the $\msf{NSL_{\oplus}}$ to $+$, variable $N_A$ could be substituted with $n_a + i - b$ to form the same attack as with $\oplus$.

Similar attacks are quite likely under the {\sf Idempotency} property as well since it too involves cancellation, although we did not find any on the $\msf{NSL_{\oplus}}$ protocol when the $\oplus$ operator is equipped with this property.

The above attack can be avoided if Msg~2 in $\msf{NSL_{\oplus}}$ is changed to 

\begin{center}
\begin{tabular}{ll}

Msg 2. $B \to A : [ [\msf{nonce}\oplus\msf{agent}, [\msf{nonce},N_A] \oplus [\msf{agent},B]],  [\msf{nonce},N_B] ]^{\to}_{\mathit{pk}(A)}$\\

\end{tabular}
\end{center}

Notice the type-tagging which is made more detailed with each  term connected with the \texttt{XOR} operator tagged individually. Msg~$\beta$.2 is then non-unifiable with Msg~$\alpha$.2 even when $i(a)$ sends Msg~$\beta$.1 as 


\begin{center}
\begin{tabular}{ll}

Msg $\beta$.1. $i(a) \to b : [ [\msf{agent}, a], [\msf{nonce}, [\msf{nonce},n_a] \oplus [\msf{agent},b] \oplus [\msf{agent},i]] ]^{\to}_{\mathit{pk}(b)}$ \\

\end{tabular}
\end{center}

since Msg~$\beta$.2 then becomes 


\begin{center}
\begin{tabular}{ll}

Msg $\beta$.2. $b \to i(a) : [ [\msf{nonce} \oplus \msf{agent}, [\msf{nonce}, [\msf{nonce},n_a] \oplus [\msf{agent},b] \oplus [\msf{agent},i] \oplus [\msf{agent},b]],$ \\ $~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~[\msf{nonce},n_b]]^{\to}_{\mathit{pk}(a)}$ \\

\end{tabular}
\end{center}

which is not unifiable with Msg~$\alpha$.2: 

\begin{center}
\begin{tabular}{ll}

Msg $\alpha$.2. $i  \to  a : [ [\msf{nonce} \oplus \msf{agent}, [\msf{nonce},n_a] \oplus [\msf{agent},i]], [\msf{nonce},n_b]]^{\to}_{\mathit{pk}(a)}$ \\

\end{tabular}
\end{center}

even after canceling the $[\msf{agent},b]$ present twice. A similar reasoning applies to {\sf Inverse} property for $\oplus$ instead of {\sf Nilpotence}.

We prove that this detailed type-tagging prevents all type-flaw attacks under monoidal theories in Appendix \ref{sa.proofs}. We consider \texttt{XOR} as a representative operator and first extend the constraint solving model accordingly. In particular, we adopt Chevalier's \cite{C-unif2004} extension for \texttt{XOR}  which extends the model by adding two new reduction rules: one that decomposes an \texttt{XOR} term on the left into its individual elements and another that composes terms on the right (the term set) into a new \texttt{XOR} term.

In this extended model, it would be only pertinent to reprove Lemma~\ref{l.well-typed} by including the \texttt{XOR} operator in the term algebra. However, unification has to consider both the standard theory in the term algebra of Def.~\ref{d.term-algebra} and the {\sf ACUN} theory of \texttt{XOR}. We consider such equational unification using the combination method of Baader and Schulz and reprove Lemma~\ref{l.well-typed} in Appendix~\ref{sa.proofs}, Lemma~\ref{la.well-typed-xor}. Consequently, we suggest the following principle:

\begin{center}
\begin{tabular}{|l|}
\hline

\parbox[3,3]{4in}{
\begin{lesson}[Detailed type-tagging]\label{le.cancel}
When message operators possess cancellation, it is prudent to follow type-tagging, in addition to component numbering. Further, the type-tagging has to be detailed, with tags for every individual term to which message operators are applied.
\end{lesson}
}\\

\hline

\end{tabular}
\end{center}


It is obvious through the examples that this principle is necessary and our proofs establish that it is sufficient.

\subsubsection*{Summary.} Our observations on the various algebraic properties we considered can be summarized in the following table with a column each for type-tagging and component numbering as to their efficacy in preventing type-flaw attacks under the considered property:

\begin{center}
\begin{tabular}{|c|c|c|}

\hline
% &  \multicolumn{2}{l|}{\bf Type tags} & \multicolumn{2}{l|}{\bf Comp  Nos}  \\ \hline
{\bf Property} &  {\em Type tags}  &  {\em Component Numbers} \\
\hline
Prefix	property		  			 		 & C  & C  \\
\hline
Homomorphism of encryptions			 & N  & N  \\
\hline
Low-Exponent RSA weakness			   & Y  & Y  \\
\hline
Associative pairing		  	 			 & Y  & N  \\
\hline
Commutative encryption		 			 & Y  & Y  \\
\hline
ACU														   & Y  & N  \\
\hline
ACU and Idempotence				 			 & Y  & U  \\
\hline
ACU and Nilpotence				 			 & Y  & N  \\
\hline
ACU and Inverse						 			 & Y  & N  \\
\hline

\end{tabular}
\end{center}

\noindent
{\bf Legend:} {\bf Y} - Yes; {\bf N} - No; {\bf C} - Conditional/Depends; {\bf U} - Unknown.



==> formal-proof.tex <==
\section{Formal proof for type-flaw attacks}\label{s.formal-proof}

In this section, we present a formal proof that non-unifiability of encryptions (which can be ensured by tagging with component numbers) prevents type-flaw attacks. 
Our proof is much simpler than \cite{HLS03}, and more importantly, allows us to easily study extrapolating the result to operators with algebraic properties. Furthermore, being a symbolic protocol model, the framework is quite flexible to include the much needed equational unification  for additional equational theories. 

We first achieve the result for the standard theory and then extend it in Section~\ref{sss.monoidal} for monoidal theories. 

\subsection{Term Alegbra}\label{ss.term-algebra}

We start off with a term algebra which has only free operators for now.

\begin{definition}[Terms]\label{d.term-algebra}
A \emph{term} is one of the following:

	 \emph{Variable} (can be an Agent, Nonce etc., that are all subsets of $\mi{Var}$);
	 \emph{Constant} (numbers 1,2,$\ldots$; name of the attacker $\epsilon$ etc.);
	 \emph{Atom} (split into sets agents, nonces etc.);
	 \emph{Pair} denoted $[t_1,t_2]$ if $t_1$ and $t_2$ are terms;
	 \emph{Public-Key} denoted $\mi{pk}(A)$ with $A$ of type Agent;
	 \emph{Shared-Key} denoted $\mi{sh}(A,B)$ with $A$ and $B$ of type Agent;
	 \emph{Asymmetric encryption} denoted $[t]^{\to}_k$ where $t$ and $k$ are terms;
	 \emph{Symmetric encryption} denoted $[t]^{\leftrightarrow}_k$ where $t$ and $k$ are terms;
	 \emph{Hash} denoted $h(t)$ where $t$ is a term;
	 \emph{Signature} denoted $\mi{Sig}_k(t)$ where $t$ is a term to be validated using the key $k$.

\end{definition}

We will often write a sequence of terms without brackets  for pairing (e.g. $[N_A,[N_B,B]]$ as $[N_A,N_B,B]$) if the brackets are contextually insignificant.
We will drop the superscript $\to$ or $\leftrightarrow$ if the mode of encryption is irrelevant. We will call encrypted subterms, hashes and signatures as \emph{Compound Terms}; we will denote them as $\mi{CT}(T)$ for a set of terms, $T$. 

We will call terms with no atoms (but only constants and variables) as {\em parametric terms}. We will call a parametric term in which some of the variables were substituted with atoms as a \emph{semi-term}. 

We will assume that the reader is familiar with the standard definitions of syntactic unification, and the most general unifier (mgu). We also provide them in Appendix~\ref{s.defs}. We will write $t \approx t'$ if $t$ and $t'$ are unifiable.

As usual, {\em subterms} are defined to capture parts of messages:

\begin{definition}[Subterm]\label{d.subterm}

Term $t$ is a \emph{subterm} of $t'$ (denoted $t \sqsubset t')$ if $t = t'$, or if $t' = [t_1, t_2]$ with $t \sqsubset t_1 \vee t \sqsubset t_2$, or if $t' = [t^{''}]_{k'}$ with $t \sqsubset t^{''}$, or if $t' = h(t^{''})$ with $t \sqsubset t^{''}$, or if $t' = \mi{Sig}_k(t^{''})$ with $t \sqsubset t^{''}$.

\end{definition}


We will denote the type of a variable $V$ as $\mi{type}(V)$. This can of course be recursively defined to define the types of complex terms as well (pair of agents, encryption of a pair of agents etc.). 

We will take advantage of naming conventions to group different sets of atoms each set with a unique type. E.g. A nonce variable $N_V$ is of type \emph{Nonce} and a nonce $n_v$ belongs to the set {\em Nonce}. This eases defining substitutions that are well-typed: We will call a substitution of an atom $x$ to a variable $X$ a ``well-typed" substitution, if $x \in \mi{type}(V)$. We will call a set of substitutions $\sigma$ as well-typed and write {\sf well-typed}$(\sigma)$ if all its members are well-typed; otherwise, we call $\sigma$ ill-typed.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%  		STRAND SPACES				%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Strands and Semi-bundles}\label{ss.strands-semib}

The protocol model is based on the strand space framework of \cite{THG98}.

\begin{definition}[Node, Strand, Protocol]\label{d.node-strand}

A \emph{node} is a tuple $\langle \mi{Sign}, \mi{Term} \rangle$ denoted $+m$ when it sends a term $m$, or $-m$ when it receives $m$. The {\em sign} of a node $n$ is denoted $\mathrm{sign}(n)$ that can be `$+$' or `$-$' and its term as $\mathrm{term}(n)$ derived from the term algebra.
A \emph{strand} is a sequence of nodes. Nodes in a strand are related by the edge $\Rightarrow$ defined such that if $n_i$ and $n_{i+1}$ belong to the same strand, then we write $n_i \Rightarrow n_{i+1}$. A \emph{parametric strand} is a strand with all parametric terms on its nodes. A {\em protocol} is a set of parametric strands.
\end{definition}

Protocol roles (or parametric strands) can be partially instantiated to produce  {\em semi-strands} containing semi-terms on nodes obtained instantiating their parametric terms, depending on the knowledge of agents concerning the variables being instantiated: A variable is instantiated to an atom if the agent to which the strand corresponds to, either creates the atom according to the protocol or knows the value ({\em e.g.} being public such as an agent name). 

We will denote the substitution of a parametric strand `$p$' by an honest agent leading to a semi-strand `$s$' as $\sigma^h_s p$ where $\sigma^h_s$ is the agent's substitution.  

For instance, role `$A$' in the Needham-Schroeder-Lowe (NSL) protocol is the parametric strand $\mi{role_A} = \langle +[N_A,A]^{\to}_{\mi{pk}(B)}, -[N_A,N_B,A]^{\to}_{\mi{pk}(A)}, +[N_B]^{\to}_{\mi{pk}(B)} \rangle$ and an agent `$a$' that plays the role could be the semi-strand \\ $\sigma^h_s role_A = \langle +[n_a,a]^{\to}_{\mi{pk}(B)}, -[n_a,N_B,a]^{\to}_{\mi{pk}(a)}, +[N_B]^{\to}_{\mi{pk}(B)} \rangle$ where $\sigma^h_s = \{ a/A,n_a/N_A \}$.

A set of semi-strands is a \emph{semi-bundle}. We will denote the set of all honest substitutions of parametric strands selected from a set $P$ leading to a semi-bundle $S$ as $S = \sigma^H_S P$. 

We will assume that honest agent substitutions leading to semi-strands are always well-typed:

\begin{assumption}\label{a.well-typed}
	Let $P$ be a protocol and $S$ be a semi-bundle such that $S = \sigma^H_S P$. Then,	$(\forall \sigma^h_s \in \sigma^H_S)(\text{\sf well-typed}(\sigma^h_s))$.	
\end{assumption}

%We will write $t \in S$ even if $(t = \text{term}(n)) \wedge (n \in s) \wedge (s \in S)$ and $t \sqsubset S$ if $(t \sqsubset t') \wedge (t' \in S)$. We will (ab)use the notation of $\mi{CT}()$ on protocols and semi-bundles as well.

We will use the relation `precedes' ($\preceq$) on stand-alone strands in semi-bundles: Let $s$ be a strand in a semi-bundle $S$. Then, $(\forall n_i, n_j \in s)(s \in S)(i \leq j \Rightarrow n_i \preceq n_j)$. 

We will abuse the notation of $CT()$ on strands, protocols and semi-bundles as well. We will write $t \in S$ even if $t$ is a term on some node of some strand of a semi-bundle $S$.

%We will denote the set of initial intruder knowledge as $\mi{IIK}$. We will assume that the intruder (or attacker) knows the names of all the agents, constants, public-keys, and its own private key, nonces, and the shared keys that is shares with other agents.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%		CONSTRAINT SOLVING			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Constraints and Satisfiability}\label{ss.constraints}

We use the constraint solving model of Millen-Shmatikov \cite{MS01} to model the penetrator\footnote{Heather et al. \cite{HLS00} used classical penetrator strands of \cite{THG98}, but the basic penetrator capabilities are same and equal in both models.}. We present both {\bf P} and $R$ in Appendix~\ref{sa.prot-model} to make the paper self-contained. We provide some formal definitions of the model here to achieve rigor in our results. We use the same terminology and notation as in \cite{MS01} in our framework and proof to maintain consistency.

The main constraint satisfaction procedure in \cite{MS01}, namely {\bf P}, first forms a constraint sequence from an interleaving of nodes belonging to strands in a semi-bundle:

\begin{definition}[Constraint sequence]\label{d.conseq}

A {\em constraint sequence} $C = \langle \text{term}(n_1)~:~T_1,\ldots,\text{term}(n_k)~:~T_k\rangle$ is from a semi-bundle $S$ with $k$ `$-$' nodes if $(\forall n)(\forall n')(\text{term}(n')~:~T_i \in C)(\text{term}(n) \in T_i)(n \preceq n')$. Further, if $i < j$ and $n_i$, $n_j$ belong to the same strand, then $n_i \preceq n_j$ and $(\forall i)(T_i \subset T_{i+1})$.

\end{definition}

A symbolic reduction rule applied to a constraint $m~:~T$ is said to ``reduce" it to another constraint $m~:~T'$ or $m'~:~T$. {\bf P} applies a set of such rules $R = \{ \mathsf{pair}, \mathsf{split},$ $\mathsf{penc}, \mathsf{senc},$ $\mathsf{sdec}, \mathsf{hash}, \mathsf{sig}, \mathsf{ksub}, \mathsf{un} \}$ to reduce a constraint sequence possibly to a ``simple" constraint sequence:%\footnote{Please refer to \cite{MS01} for full details on {\bf P} and {\bf R}.}.

\begin{definition}[Simple constraint sequence]\label{d.simplecons}

A constraint $m~:~T$ is a {\em simple constraint} if $m$ is a variable. A constraint sequence $C$ is a {\em simple constraint sequence} if every constraint in $C$ is a simple constraint.

\end{definition}

The possibility of forming bundles from a given semi-bundle can be determined by testing if constraint sequences from it are satisfiable:

\begin{definition}[Satisfiability]\label{d.satisfiable}

A constraint is {\em satisfiable} if a sequence of reduction rule application from $R$ result in a simple constraint. A constraint sequence $C$ is {\em satisfiable} if every constraint in the sequence is satisfiable. Further, the initially empty substitution $\sigma$ is said to satisfy $C$, denoted $\sigma \vdash C$. 

%A minus ($-$) node is \emph{realizable} if the corresponding constraint is satisfiable. A semi-bundle $S$ which $C$ is from, is {\em realizable} to a bundle if $C$ is satisfiable.

\end{definition}

We will assume that the left side of a constraint is never a pair where rule ({\em un}) is applied to unify terms. It can be proved that any attack without this assumption can be realized under it as well.

Violations of trace properties such as secrecy and authentication can be embedded in a semi-bundle so that a satisfiable constraint sequence from the semi-bundle points to an attack. Using this concept, we define a type-flaw attack: 

\begin{definition}[Type-flaw attacks]\label{d.type-flaw}

A {\em type-flaw attack} exists on a semi-bundle $S$ if a constraint sequence $C$ from $S$ is satisfiable with an ill-typed substitution, but not with a well-typed substitution. i.e. $(\exists \sigma)(\sigma \vdash C) \Rightarrow (\nexists \sigma^{'})((\sigma' \vdash C) \wedge (\text{\sf well-typed}(\sigma^{'})))$. 

\end{definition}
 
 
\subsection{Main requirement --- Non-Unifiability of Terms}\label{ss.NUT}

We will now state our main requirement on protocol messages  which states that textually distinct encryptions should be non-unifiable:

\begin{definition}[{\sf NUT}]\label{d.Mu-NUT}

Let $P$ be a protocol. Then $P$ is $\msf{NUT}$-Satisfying iff $(\forall t_1 \in CT(P))(\forall t_2 \in CT(P))(t_1 \neq t_2 \Rightarrow t_1 \not\approx t_2).$

\end{definition}

It can be easily seen that {\sf NUT} is achieved by following the same suggestion as Heather et al. to place component numbers as the beginning element of concatenations inside all distinct compound terms in a protocol. E.g.  $[1,[N_A,A]]^{\to}_{\mi{pk}(B)}$, $[2,[N_A,[3,N_B,A]^{\leftrightarrow}_{\mi{sh}(A,B)}]]^{\leftrightarrow}_{\mi{sh}(B,S)}$,   etc.

%Notice that an \textsf{NUT}-Satisfying protocol has {\em EV-Freedom} \cite{Mill03} naturally so the results apply equally well even with an explicit decryption operator for symmetric key encryption. It is possible {\sf NUT} captures {\em pk-freedom} and/or {\em structure} so that the same holds for asymmetric key encryption as well \cite{LM05}.

\subsection{Main result}\label{ss.main-result}

We first prove three simple lemmas. The proofs can be found in Appendix~\ref{sa.proofs}. The first lemma proves that the reduction rules corresponding to standard attacker inferences always add existing subterms to the term set of the original constraint:

\begin{lemma}[Rules in $R$ always produce subterms]\label{l.produce-subt}

	If a rule in $R$ is applied to a constraint $c = m~:~T$ such that $c$ is reduced to $m~:~T \cup t$, then $t \sqsubset T$.

\end{lemma}

The second lemma proves that inserting distinct constants into distinct parametric terms of a protocol ensures that the terms remain non-unifiable even after instantiated to semi-terms:

\begin{lemma}[NUT guarantees non-unifiability in semi-bundles]\label{l.nut}

	If two terms $t_1$, $t_2$ in a semi-bundle $S$ from an \textsf{NUT}-Satisfying protocol  $P$ are such that $t_1 = \sigma^h_a t'_1$ and $t_2 = \sigma^h_b t'_2$ where $\sigma^h_a \neq \sigma^h_b$ and $\{ \sigma^h_a, \sigma^h_b \} \subseteq \sigma^H_S$ and $S = \sigma^H_S P$, $t'_1, t'_2 \in P$, and $t'_1 \neq t'_2$, then $t_1 \not\approx t_2$.

\end{lemma}

The final lemma proves that unification in a semi-bundle from a {\sf NUT}-Satisfying protocol always returns well-typed unifiers.

\begin{lemma}[Necessarily well-typed unifiers]\label{l.well-typed}

 Let $S$ be a semi-bundle from a {\sf NUT}-Satisfying protocol and let $t, t' \in S$ for a semi-bundle $S$ such that $t = \sigma^h_{s} x$ and $t' = \sigma^h_{s'} x$ for some $s, s' \in S$. Then, $\text{\sf well-typed}(\tau)$ where $\text{mgu}(t,t') = \tau$.

\end{lemma}

We now use these lemmas and the definition of type-flaw attacks in Def.~\ref{d.type-flaw} to achieve our main result. The intuition is simple: the two reduction rules that affect the attacker substitution on satisfiable constraint sequences are identified. The above lemmas are then used to show that both, and importantly, the more commonly used rule of the two, namely {\sf un}, always produces a well-typed unifier as long as the constraint sequence is from a semi-bundle which in turn was from a {\sf NUT}-Satisfying protocol. Since type-flaw attacks occur only when ill-typed substitutions satisfy constraint sequences, this proves the impossibility of such attacks.

\begin{theorem}[\textsf{NUT} prevents type-flaw attacks]\label{t.type-flaw}

Let $P$ be a $\msf{NUT}$-Satisfying protocol  and $S = \sigma^H_S P$. Let $C$ be from $S$. Then, $(\sigma \vdash C) \Rightarrow (\exists \sigma')((\sigma' \vdash C) \wedge (\text{\sf well-typed}(\sigma')))$.

\end{theorem}

\begin{proof}

If $\sigma$ satisfies $C$, then rules from $R$ have been used to reduce it to a simple constraint sequence, $C'$. The only rules that can change $\sigma$ are ($\mi{un}$) and ($\mi{ksub}$). ($\mi{ksub}$) makes a well-typed substitution since it unifies a term with the attacker's public-key which is of the same type.

So, we have to now prove that if $m~:~T \cup t \in C$, and $m \approx t$ with $\text{mgu}(m,t) = \tau$, then $\text{\sf well-typed}(\tau)$. 

\begin{itemize}

		\item Now $m$ is a subterm of $S$ and from 												Lemma~\ref{l.produce-subt}, we have that $t$ 								has to be a subterm of $S$, so let $m \approx t$ 						where $m = \sigma^h_s x$ and $t = \sigma^h_{s'} 						y$ for some $s, s' \in S$.  

		\item Since $P$ is \textsf{NUT}-Satisfying, from 									Lemma~\ref{l.nut} if $x \neq y$, then $m 										\not\approx t$, a contradiction. Hence, $x$ has 						to equal $y$.

		\item From Lemma~\ref{l.well-typed} we can now conclude 					that $\tau =\text{mgu}(\sigma^h_s x,\sigma^h_{s'} 					x)$ is necessarily well-typed.

\end{itemize}

Since initially $\sigma$ is empty, using induction on each constraint of the sequence, we can conclude that $\sigma$ is well-typed.


\end{proof}





==> type-flaws.tex <==
\section{Tagging prevents type-flaw attacks under \texttt{XOR}}\label{s.type-flaws}

\input{type-flaw-ex.tex}

\input{type-flaw-proof.tex}



